Deep Generative Models for Ultra-High Granularity Particle Physics Detector Simulation: A Voyage From Emulation to Extrapolation

Simulating ultra-high-granularity detector responses in Particle Physics represents a critical yet computationally demanding task. This thesis aims to overcome this challenge for the Pixel Vertex Detector (PXD) at the Belle II experiment, which features over 7.5M pixel channels-the highest spatial resolution detector simulation dataset ever analysed with generative models. This thesis starts off by a comprehensive and taxonomic review on generative models for simulating detector signatures. Then, it presents the Intra-Event Aware Generative Adversarial Network (IEA-GAN), a new geometry-aware generative model that introduces a relational attentive reasoning and Self-Supervised Learning to approximate an "event" in the detector. This study underscores the importance of intra-event correlation for downstream physics analyses. Building upon this, the work drifts towards a more generic approach and presents YonedaVAE, a Category Theory-inspired generative model that tackles the open problem of Out-of-Distribution (OOD) simulation. YonedaVAE introduces a learnable Yoneda embedding to capture the entirety of an event based on its sensor relationships, formulating a Category theoretical language for intra-event relational reasoning. This is complemented by introducing a Self-Supervised learnable prior for VAEs and an Adaptive Top-q sampling mechanism, enabling the model to sample point clouds with variable intra-category cardinality in a zero-shot manner. Variable Intra-event cardinality has not been approached before and is vital for simulating irregular detector geometries. Trained on an early experiment data, YonedaVAE can reach a reasonable OOD simulation precision of a later experiment with almost double luminosity. This study introduces, for the first time, the results of using deep generative models for ultra-high granularity detector simulation in Particle Physics.

==> pages/anhang.tex <==
\begin{appendix}


\chapter{Der erste Anhang}

Hier steht der erste Anhang.


\chapter{Zweiter Anhang}

Hier kommt der zweite Anhang.


\end{appendix}


==> pages/titleblatt_2.tex <==
\begin{titlepage}   
   {\sffamily
    \vspace*{\stretch{1}}
    {\parindent0cm
    \rule{\linewidth}{.7ex}}  
  \begin{flushright}
    \vspace*{\stretch{1}}
    {\LARGE \bfseries \baselineskip=24pt \getSubtitle{}}
    
    %\vspace*{2ex}
    %{\Large \bfseries \getSubtitle{}}
    
    \vspace*{\stretch{1}}
    {\large\bfseries \getAuthor{}}
    
    \vspace*{\stretch{1}}
  \end{flushright}
    \rule{\linewidth}{.7ex}
    \vspace*{\stretch{3}}
    
  \begin{center}
    {\large
     Dissertation\\
     der Fakultät für Physik\\
     der Ludwig-Maximilians-Universität\\
     München
     
    \vspace*{\stretch{1}}    
     vorgelegt von\\
     \getAuthor{}\\
     aus \getPlaceOfBirth{}
     
    \vspace*{\stretch{2}}   
     \getPrintLocation{}, den \getSubmissionDate{}
     }
  \end{center}
   }
\end{titlepage}
